DIFT: Dynamic Iterative Field Transforms for Memory Efficient Optical Flow

Recent advancements in neural network-based optical flow estimation often come with prohibitively high computational and memory requirements, presenting challenges in their model adaptation for mobile and low-power use cases. In this paper, we introduce a lightweight low-latency and memory-efficient model, Dynamic Iterative Field Transforms (DIFT), for optical flow estimation feasible for edge applications such as mobile, XR, micro UAVs, robotics and cameras. DIFT follows an iterative refinement framework leveraging variable resolution of cost volumes for correspondence estimation. We propose a memory efficient solution for cost volume processing to reduce peak memory. Also, we present a novel dynamic coarse-to-fine cost volume processing during various stages of refinement to avoid multiple levels of cost volumes. We demonstrate first real-time cost-volume based optical flow DL architecture on Snapdragon 8 Gen 1 HTP efficient mobile AI accelerator with 32 inf/sec and 5.89 EPE (endpoint error) on KITTI with manageable accuracy-performance tradeoffs.

==> Previous/icassp_rebuttal.tex <==


We sincerely thank all the reviewers for their constructive feedback. We are pleased that some reviewers found that our consistency strategies are well-motivated and that some reviewers agreed that our method convincingly performs better than the previous baseline method.

Here we try our best to respond to all the questions from the reviewers.

\newcommand\rone{{\textcolor{red}{\textbf{\mbox{R1}}}}}

\section{Rebuttal}

\begin{itemize}

    \item \textbf{(R1)} Comparision to RAFT?
        Reviewer Comment: Peak memory comparisons be presented in a table with the proposed scheme and other alternative learning based optical flow implementations
    \item \textbf{R2 comments}
    \item Description of Encoder \& Update block clearly
    \item Dataset Description
    \item Hardware Platform: 
        \subitem clarify HTP is mobile AI accelerator within 8Gen1, when power/efficiency is not a constraint can run on GPU or other modules of snapdragon
    \item radius = 3, why not other radius
    \item Other Datasets?
    \item writing: typos & formatting.
\end{itemize}

\subsection{Comparison to RAFT:}

Sorry for any confusion, but we would like re-iterate that RAFT as it is not suitable to run on-mobile platform because even memory efficient version needs significant memory. 

In case of Sintel, even after 16x downsampling instead of 8x (for  efficient latency), and \textbf{radius =  3}, we will have 440 x 1024 original image down-sampled to $28 \times 65 \times (2 \times (radius = 3+1)) = $

==> experiments.tex <==

\section{Experiments}
\textbf{Datasets:} 

\subsection{Experimental Setup}


\subsection{Design Questions/Ablation Study} %% Ablation Study

\begin{itemize}
    \item Affect of number of cost volume resolutions
    \item Coarse2fine vs single-level cost volume
        \subitem weight sharing
    \item Affect of Cost-volume resolution
    \item Affect of number of iterations
    \item Affect of Channel dimension
    \item model-distillation for better inference latency vs performance?
\end{itemize}


\subsection{Results}

% \begin{itemize}
%     \item model-distillation for better inference latency vs performance?
%     \item Adding more capacity to process look up output? especially for radius = 7/more channels..
%     \item multi-scale encoder?
%     \item Position encoding vs prev. flow concat for skip connection of look up operation?
    
%     \item \textbf{For potential CVPR Submission?}
%     %% combining various recent works into a single high performing architecture with extended ablations.
%     \subitem Global vs Local (ablation)
%     \subitem Patch based vs pixel level cost volume 
%     \subitem start with patch level correspondence then pixel level correspondence
%     \subitem Features(e.g. from GMFlow i.e. cross attention) vs matching importance for O.F i.e. if we start with good features does correspondence get easier, and what should be training pipeline for low latency
%     \subitem 
    
% \end{itemize}

%% include other design questions here


==> method.tex <==
\section{Mobile RAFT} %% Our Solution


% \subsection{Proposed Network}
% Here we describe few core modifications and final architecture properties. Overall aim to find simplest possible RAFT based architecture for Optical Flow or Stereo for mobile applications.
% \begin{itemize}
%     \item JiT version of lookup, i.e. local processing of cost volume + tiling
%     \item Coarse to fine look up with single level cost volume based iterative refinement
%     \item \textit{Replacing grid sampling with bi-linear shift with only element wise operations}
%     \item Skip connections of look up output, i.e., preserving previous look up output to minimize number of look up operations \& also have global cost volume information.
%     \item Resolution dependent weight sharing during for iterative refinement.
% \end{itemize}

\subsection{Memory efficient Lookup}

\subsection{Coarse to Fine Lookup}

To capture large motion, for initial iterations of network we adapt a coarse resolution for cost volume such that the network can have better initialization for further refinement. Once we assume we have a reasonable initialization of flow we adapt finer resolutions of cost volume

\subsection{Replacing Grid Sampling with Bilinear shift}

\subsection{Proposed Architecture}
Our architecture is inspired by RAFT but as stated earlier we make various changes to make the overall network memory and computationally efficient to achieve good performance within extreme low compute and memory constraints.

We performed extensive experiments to understand purpose and effectiveness of different components of  modern optical flow architechtures satisfying our low compute constraints. Based on overall results as later discussed in experimental section.

We propose our overall architecture where we only choose a single level cost volume in an iterative refinement scheme. We adopt Coarse to fine lookup with in single level cost volume as discussed  earlier. In addition as we have varying receptive fields w.r.t cost volume we do not share parameters of refinement/update block across all iterations but parameter sharing is dependent on cost volume resolution. We choose a very efficient network with xx channels in the encoder, xx iterations, xx down sampling of cost volume resolution.
\subsubsection{Training}
Fine tuning from large iterations to fewer iterations during training. To capture good encoder and update block features as initialization and from a good initialization fine-tune model further for reducing number of iterations. As we can interpret number of iterations as number of steps required to converge to fixed point, it is  important to allow finer steps to get close to fixed point but once we learn features and are converging to fixed point, we can potentially increase step size along paths as now training is better guided from a strong initialization.

